Layered Insights: Generalizable Analysis of Authorial Style by Leveraging All Transformer Layers

We propose a new approach for the authorship attribution task that leverages the various linguistic representations learned at different layers of pre-trained transformer-based models. We evaluate our approach on three datasets, comparing it to a state-of-the-art baseline in in-domain and out-of-domain scenarios. We found that utilizing various transformer layers improves the robustness of authorship attribution models when tested on out-of-domain data, resulting in new state-of-the-art results. Our analysis gives further insights into how our model's different layers get specialized in representing certain stylistic features that benefit the model when tested out of the domain.

==> tables/results_modernbert.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{llrrrrrr}
\multicolumn{2}{c}{\textbf{}} & \multicolumn{6}{c}{\textbf{Training Dataset}}\\
\cmidrule{3-8}
\multirow{2}{*}{\textbf{Evaluation Dataset}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Reddit}} & \multicolumn{2}{c}{\textbf{Amazon}} & \multicolumn{2}{c}{\textbf{Fanfic}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
  & & \textbf{R@8} & \textbf{MRR} & \textbf{R@8} & \textbf{MRR} & \textbf{R@8} & \textbf{MRR} \\
\midrule
\multirow{2}{*}{\textbf{Reddit}} 
        & MultiLUAR & \cellcolor{gray!20}70.37 & \cellcolor{gray!20}55.49 & \textbf{26.77} & \textbf{17.85} & \textbf{16.26} & \textbf{10.86} \\
        & LUAR      & \cellcolor{gray!20}\textbf{72.29} & \cellcolor{gray!20}\textbf{56.89} & 19.88 & 12.70 & 10.95 & 6.81 \\
\midrule
\multirow{2}{*}{\textbf{Amazon}} 
        & MultiLUAR & \textbf{87.65} & \textbf{80.79} & \cellcolor{gray!20}\textbf{96.70} & \cellcolor{gray!20}\textbf{92.07} & \textbf{63.52} & \textbf{50.65} \\
        & LUAR      & 86.38 & 78.69 & \cellcolor{gray!20}95.90 & \cellcolor{gray!20}89.12 & 32.39 & 22.14 \\
\midrule
\multirow{2}{*}{\textbf{Fanfic}} 
        & MultiLUAR & \textbf{46.32} & \textbf{35.83} & \textbf{39.71} & \textbf{29.01} & \cellcolor{gray!20}56.50 & \cellcolor{gray!20}46.46 \\
        & LUAR      & 42.41 & 31.79 & 27.86 & 18.64 & \cellcolor{gray!20}\textbf{58.47} & \cellcolor{gray!20}\textbf{47.67} \\
\bottomrule
\end{tabular}
\caption{Evaluation results comparing MultiLUAR and LUAR models built on the ModernBERT base. Results are shown across all evaluation datasets with in-domain results highlighted in gray. Higher values between the two models are bolded.}
\label{modernbert-results}
\end{table*}

